Two Deep Learning Solutions for Automatic Blurring of Faces in Videos

The widespread use of cameras in everyday life situations generates a vast amount of data that may contain sensitive information about the people and vehicles moving in front of them (location, license plates, physical characteristics, etc). In particular, people's faces are recorded by surveillance cameras in public spaces. In order to ensure the privacy of individuals, face blurring techniques can be applied to the collected videos. In this paper we present two deep-learning based options to tackle the problem. First, a direct approach, consisting of a classical object detector (based on the YOLO architecture) trained to detect faces, which are subsequently blurred. Second, an indirect approach, in which a Unet-like segmentation network is trained to output a version of the input image in which all the faces have been blurred.

==> makefile <==
# makefile for IPOL articles
# to be used with the IPOL LaTeX class verson 0.4

DOC	= article
TEX	= $(wildcard *.tex)
BIB	= $(wildcard *.bib)
LATEX	= pdflatex -interaction nonstopmode -halt-on-error
BIBTEX	= bibtex
DPILR	= 96
PDFLR	= ps2pdf -dCompatibilityLevel=1.4 \
		-dEmbedAllFonts=true \
		-dAutoRotatePages=/None \
		-dPDFSETTINGS=/screen \
		-dColorConversionStrategy=/LeaveColorUnchanged \
		-dColorImageResolution=$(DPILR) \
		-dGrayImageResolution=$(DPILR) \
		-dMonoImageResolution=$(DPILR)

default :	pdf
pdf:	$(DOC).pdf
all:	$(DOC).pdf $(DOC)_lr.pdf

# LaTeX->PDF compilation
%.pdf	: %.tex $(TEX) $(BIB)
	-$(LATEX) -draftmode $*.tex >/dev/null 2>&1
	-$(BIBTEX) $*.aux
	-$(LATEX) -draftmode $*.tex >/dev/null 2>&1
	$(LATEX) $*.tex

# PDF filtering
%_lr.pdf	: %.pdf %.info
	$(PDFLR) $< $@
	pdftk $@ multibackground lr_header.pdf output $@.tmp \
		&& mv -f $@.tmp $@
	pdftk $@ update_info $*.info output $@.tmp \
		&& mv -f $@.tmp $@
	qpdf --linearize --stream-data=compress $@ $@.tmp \
		&& mv -f $@.tmp $@

# metadata
%.info	: %.pdf
	pdftk $< dump_data output $@

# cleanup
clean	:
	$(RM) $(DOC).aux $(DOC).log $(DOC).out
	$(RM) $(DOC).blg $(DOC).bbl $(DOC).toc
	$(RM) $(DOC).info
distclean	: clean
	$(RM) $(DOC).pdf $(DOC)_lr.pdf

.PHONY	: pdf all clean distclean

